Detecting Multi-Parameter Constraint Inconsistencies in Python Data Science Libraries

Modern AI- and Data-intensive software systems rely heavily on data science and machine learning libraries that provide essential algorithmic implementations and computational frameworks. These libraries expose complex APIs whose correct usage has to follow constraints among multiple interdependent parameters. Developers using these APIs are expected to learn about the constraints through the provided documentations and any discrepancy may lead to unexpected behaviors. However, maintaining correct and consistent multi-parameter constraints in API documentations remains a significant challenge for API compatibility and reliability. To address this challenge, we propose MPDetector, for detecting inconsistencies between code and documentation, specifically focusing on multi-parameter constraints. MPDetector identifies these constraints at the code level by exploring execution paths through symbolic execution and further extracts corresponding constraints from documentation using large language models (LLMs). We propose a customized fuzzy constraint logic to reconcile the unpredictability of LLM outputs and detects logical inconsistencies between the code and documentation constraints. We collected and constructed two datasets from four popular data science libraries and evaluated MPDetector on them. The results demonstrate that MPDetector can effectively detect inconsistency issues with the precision of 92.8%. We further reported 14 detected inconsistency issues to the library developers, who have confirmed 11 issues at the time of writing.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> content/02.examples.tex <==
\section{Examples}\label{sec:eg}
In this section, we will use two examples to illustrate inconsistencies between API documentation and corresponding code caused by multi-parameter interdependence. Both of them come from real-world open source data science libraries on GitHub. We show these two inconsistencies not only since they represent the typical CDI issues in API documentation, but also because they were all successfully detected by \tool. In general, there are two types of constraints:
\begin{enumerate}
    \item \textbf{Explicit Constraint.} Explicit constraints refer to the clear specification of two interrelated parameters and the relationship between them when specifying constraints in the documentation.
    \item \textbf{Implicit Constraint.} Implicit constraint refers to an unstated or indirectly
    implied relationship between two interrelated parameters, where the constraint is understood
    through context or convention rather than explicitly specification.
\end{enumerate}


\subsection{Example 1: Explicit Constraint}\label{sec:eg1}
The first example comes from \texttt{statsmodels}~\cite{github:statsmodels}, which provides a complement to \texttt{scipy} for statistical computations including descriptive statistical and estimation and inference for statistical models. Statsmodels has around 10K stars on GitHub and is actively maintained. Figure~\ref{fig:eg1} illustrates an inconsistency caused by an explicit constraint from the class \textit{AutoReg}. The highlighted sections indicate the locations where constraints are described in the documentation and where they are checked in the code. As mentioned in the description, the trigger condition for the warning is that ``trend is not n, \textbf{and} seasonal is not False''. However, it is apparent that the actual code logic being executed is an \textbf{or} operation rather than an \textbf{and} operation. Therefore, correct documentation should change ``and'' to ``or''.


\begin{figure*}[t]
    \begin{subfigure}{\linewidth}
        \begin{tcolorbox}[colback=Emerald!10,colframe=cyan!40!black,title=\textbf{Constraint description of \texttt{trend} and \texttt{seasonal} in class \texttt{AutoReg}}]
            {\sffamily \textbf{> deterministic: } DeterministicProcess
            \\
            A deterministic process. If provided, trend and seasonal are ignored. \colorbox{blue!20}{A warning is raised if} \colorbox{blue!20}{trend is not "n" and seasonal is not False.}}
        \end{tcolorbox}
        \label{fig:eg1-doc}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
\begin{tcolorbox}[colback=Salmon!20, colframe=Salmon!90!Black,title=\textbf{Corresponding code snippet in class \texttt{AutoReg}}]
\begin{lstlisting}[escapechar=@]
class AutoReg(tsa_model.TimeSeriesModel):
    def __init__(...):
        if deterministic is not None and @\colorbox{blue!20}{(self.trend != "n" or self.seasonal)}@:
            warnings.warn('When using deterministic, trend must be "n" 
                and seasonal must be False.', SpecificationWarning, stacklevel=2)
\end{lstlisting}
\end{tcolorbox}
        \label{fig:eg1-code}
    \end{subfigure}
    \caption{Examples of an explicit constraint from \Code{Statsmodels}.}
    \label{fig:eg1}
\end{figure*}





\subsection{Example 2: Implicit Constraint}\label{sec:eg2}
The second example comes from \texttt{scikit-learn}~\cite{github:scikit}, which is a widely-used (25K stars on GitHub) open-source machine learning library in Python, designed to offer simple and efficient tools for data mining and data analysis. Figure~\ref{fig:eg2} displays an inconsistency caused by an implicit constraint from the class \textit{SpectralClustering}. It is evident that the highlighted part of the documentation only explicitly mentions one parameter \textit{affinity}, however, it lacks the subject ``gamma''. More importantly, ``ignore'' is not a specific value but rather an execution logic which means when the parameter \textit{affinity} is set to \textit{nearest\_neighbors}, the parameter \textit{gamma} will not be used. Whereas, above constraint does not fully reflect the code's behavior. According to the code snippet, ``gamma'' is not only ignored within the \textit{nearest\_neighbors} branch, but also ignored within the \textit{precomputed\_nearest\_neighbors} and \textit{precomputed} branches. This indicates that the constraint is incomplete and demonstrates a form of inconsistency.

For this type of implicit constraint, traditional pattern-based tools not only struggle to accurately extract the constraints but also fall short of detecting inconsistencies. Hence, on one hand, we tailor an output format that incorporates fuzzy words, and adopt few-shot learning to teach the LLM on how to generate this format (See details in Section~\ref{sec:llm}). In this case, it should be ``(affinity = "nearest\_neighbors") $\rightarrow$ (gamma = "ignore")''. On the other hand, we define a special predicate ``ignore(x)'' to indicate that a variable \textit{x} is ignored. (See details in Section~\ref{sec:fuzzword}).


\begin{figure*}[t]
    \begin{subfigure}{\linewidth}
        \begin{tcolorbox}[colback=Emerald!10,colframe=cyan!40!black,title=\textbf{Constraint description of \texttt{gamma} and \texttt{affinity} in class \texttt{SpectralClustering}}]
            {\sffamily \textbf{> gamma} : float, default=10
            \\
            Kernel coefficient for rbf, poly, sigmoid, laplacian and chi2 kernels. \colorbox{blue!20}{\textbf{Ignored for}} \colorbox{blue!20}{\textbf{affinity="nearest\_neighbors".}}}
        \end{tcolorbox}
        \label{fig:eg2-doc}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
\begin{tcolorbox}[colback=Salmon!20, colframe=Salmon!90!Black,title=\textbf{Corresponding code snippet in class \texttt{SpectralClustering}}]
\begin{lstlisting}[escapechar=@]
class SpectralClustering(ClusterMixin, BaseEstimator):
    def fit(self, X, y=None):
        if @\colorbox{blue!20}{self.affinity == "nearest\_neighbors"}@:
            ...
        elif @\colorbox{blue!20}{self.affinity == "precomputed\_nearest\_neighbors"}@:
            ...
        elif @\colorbox{blue!20}{self.affinity == "precomputed"}@:
            ...
        else:
            params = self.kernel_params
            if params is None:
                params = {}
            if not callable(self.affinity):
            @\colorbox{blue!20}{params["gamma"] = self.gamma}@
                params["degree"] = self.degree
                params["coef0"] = self.coef0
\end{lstlisting}
\end{tcolorbox}
        \label{fig:eg2-code}
    \end{subfigure}
    \caption{Examples of implicit constraint from \texttt{Scikit-learn}.}
    \label{fig:eg2}
\end{figure*}

